Parameter estimation of high-dimensional linear differential equations

We study the problem of estimating the coefficients in linear ordinary differential equations (ODE's) with a diverging number of variables when the solutions are observed with noise. The solution trajectories are first smoothed with local polynomial regression and the coefficients are estimated with nonconcave penalty proposed by \cite{fan01}. Under some regularity and sparsity conditions, we show the procedure can correctly identifies nonzero coefficients with probability converging to one and the estimators for nonzero coefficients have the same asymptotic normal distribution as they would have when the zero coefficients are known and the same two-step procedure is used. Our asymptotic results are valid under the misspecified case where linear ODE's are only used as an approximation to nonlinear ODE's, and the estimates will converge to the coefficients of the best approximating linear system. From our results, when the solution trajectories of the ODE's are sufficiently smooth, the parametric $\sqrt{n}$ rate is achieved even though nonparametric regression estimator is used in the first step of the procedure. The performance of the two-step procedure is illustrated by a simulation study as well as an application to yeast cell-cycle data.

==> papers <==
@article{
abramovich04,
   Author = {Abramovich, F. and Amato, U. and Angelini, C.},
   Title = {On optimality of Bayesian wavelet estimators},
   Journal = {Scandinavian Journal of Statistics},
   Volume = {31},
   Number = {2},
   Pages = {217-234},
      Year = {2004} }



@article{
abramovich06,
   Author = {Abramovich, F. and Benjamini, Y. and Donoho, D. L. and Johnstone, I. M.},
   Title = {Adapting to unknown sparsity by controlling the false discovery rate},
   Journal = {Annals of Statistics},
   Volume = {34},
   Number = {2},
   Pages = {584-653},
      Year = {2006} }



@article{
abramovich98,
   Author = {Abramovich, F. and Sapatinas, T. and Silverman, B. W.},
   Title = {Wavelet thresholding via a Bayesian approach},
   Journal = {Journal of the Royal Statistical Society Series B-Statistical Methodology},
   Volume = {60},
   Pages = {725-749},
   Note = {Part 4},
      Year = {1998} }



@article{
andrieu05,
   Author = {Andrieu, C. and Moulines, E. and Priouret, P.},
   Title = {Stability of stochastic approximation under verifiable conditions},
   Journal = {Siam Journal on Control and Optimization},
   Volume = {44},
   Number = {1},
   Pages = {283-312},
      Year = {2005} }



@article{
bansal06,
   Author = {Bansal, M. and Della Gatta, G. and di Bernardo, D.},
   Title = {Inference of gene regulatory networks and compound mode of action from time course gene expression profiles},
   Journal = {Bioinformatics},
   Volume = {22},
   Number = {7},
   Pages = {815-822},
      Year = {2006} }



@article{
barron99,
   Author = {Barron, A. and Schervish, M. J. and Wasserman, L.},
   Title = {The consistency of posterior distributions in nonparametric problems},
   Journal = {Annals of Statistics},
   Volume = {27},
   Number = {2},
   Pages = {536-561},
      Year = {1999} }



@article{
bickel88,
   Author = {Bickel, P. J. and Ritov, Y.},
   Title = {ESTIMATING INTEGRATED SQUARED DENSITY DERIVATIVES - SHARP BEST ORDER OF CONVERGENCE-ESTIMATES},
   Journal = {Sankhya-the Indian Journal of Statistics Series A},
   Volume = {50},
   Pages = {381-393},
   Note = {Part 3},
      Year = {1988} }



@article{
biegler86,
   Author = {Biegler, L. T. and Damiano, J. J. and Blau, G. E.},
   Title = {NONLINEAR PARAMETER-ESTIMATION - A CASE-STUDY COMPARISON},
   Journal = {Aiche Journal},
   Volume = {32},
   Number = {1},
   Pages = {29-45},
      Year = {1986} }



@article{
bishop98,
   Author = {Bishop, Christopher M. and Svensen, Markus and Williams, Christopher K. I.},
   Title = {GTM: The Generative Topographic Mapping},
   Journal = {Neural Computation},
   Volume = {10},
   Number = {1},
   Pages = {215-234},
      Year = {1998} }



@article{
blackwell62,
   Author = {Blackwell, D. and Dubins, L.},
   Title = {Merging of opinions with increasing information},
   Journal = {Annals of Mathematical Statistics},
   Volume = {33},
   Pages = {882-886},
      Year = {1962} }



@article{
brown96,
   Author = {Brown, L. D. and Low, M. G.},
   Title = {Asymptotic equivalence of nonparametric regression and white noise},
   Journal = {Annals of Statistics},
   Volume = {24},
   Number = {6},
   Pages = {2384-2398},
      Year = {1996} }



@article{
cappe04,
   Author = {Cappe, O. and Guillin, A. and Marin, J. M. and Robert, C. P.},
   Title = {Population Monte Carlo},
   Journal = {Journal of Computational and Graphical Statistics},
   Volume = {13},
   Number = {4},
   Pages = {907-929},
      Year = {2004} }



@article{
chen05,
   Author = {Chen, K. C. and Wang, T. Y. and Tseng, H. H. and Huang, C. Y. F. and Kao, C. Y.},
   Title = {A stochastic differential equation model for quantifying transcriptional regulatory network in Saccharomyces cerevisiae},
   Journal = {Bioinformatics},
   Volume = {21},
   Number = {12},
   Pages = {2883-2890},
      Year = {2005} }



@article{
delyon99,
   Author = {Delyon, B. and Lavielle, V. and Moulines, E.},
   Title = {Convergence of a stochastic approximation version of the EM algorithm},
   Journal = {Annals of Statistics},
   Volume = {27},
   Number = {1},
   Pages = {94-128},
      Year = {1999} }



@article{
diaconis86,
   Author = {Diaconis, P. and Freedman, D.},
   Title = {On the Consistency of Bayes Estimates},
   Journal = {Annals of Statistics},
   Volume = {14},
   Number = {1},
   Pages = {1-26},
      Year = {1986} }



@article{
doksum95,
   Author = {Doksum, K. and Samarov, A.},
   Title = {Nonparametric estimation of global functionals and a measure of the explanatory power of covariates in regression},
   Journal = {Annals of Statistics},
   Volume = {23},
   Number = {5},
   Pages = {1443-1473},
      Year = {1995} }



@article{
donoho94,
   Author = {Donoho, D. L. and Johnstone, I. M.},
   Title = {Ideal Spatial Adaptation by Wavelet Shrinkage},
   Journal = {Biometrika},
   Volume = {81},
   Number = {3},
   Pages = {425-455},
      Year = {1994} }



@article{
donoho95a,
   Author = {Donoho, D. L. and Johnstone, I. M.},
   Title = {Adapting to unknown smoothness via wavelet shrinkage},
   Journal = {Journal of the American Statistical Association},
   Volume = {90},
   Number = {432},
   Pages = {1200-1224},
      Year = {1995} }



@article{
donoho98,
   Author = {Donoho, D. L. and Johnstone, I. M.},
   Title = {Minimax estimation via wavelet shrinkage},
   Journal = {Annals of Statistics},
   Volume = {26},
   Number = {3},
   Pages = {879-921},
      Year = {1998} }



@article{
donoho95b,
   Author = {Donoho, D. L. and Johnstone, I. M. and Kerkyacharian, G. and Picard, D.},
   Title = {Wavelet Shrinkage - Asymptopia},
   Journal = {Journal of the Royal Statistical Society Series B-Methodological},
   Volume = {57},
   Number = {2},
   Pages = {301-337},
      Year = {1995} }



@article{
donoho96,
   Author = {Donoho, D. L. and Johnstone, I. M. and Kerkyacharian, G. and Picard, D.},
   Title = {Density estimation by wavelet thresholding},
   Journal = {Annals of Statistics},
   Volume = {24},
   Number = {2},
   Pages = {508-539},
      Year = {1996} }



@article{
douc07,
   Author = {Douc, R. and Guillin, A. and Marin, J. M. and Robert, C. P.},
   Title = {Convergence of adaptive mixtures of importance sampling schemes},
   Journal = {Annals of Statistics},
   Volume = {35},
   Number = {1},
   Pages = {420-448},
   Note = {Douc, R. Guillin, A. Marin, J.-M. Robert, C. P.},
      Year = {2007} }



@article{
efron04,
   Author = {Efron, B. and Hastie, T. and Johnstone, I. and Tibshirani, R.},
   Title = {Least angle regression},
   Journal = {Annals of Statistics},
   Volume = {32},
   Number = {2},
   Pages = {407-451},
      Year = {2004} }



@article{
fan01,
   Author = {Fan, J. Q. and Li, R. Z.},
   Title = {Variable selection via nonconcave penalized likelihood and its oracle properties},
   Journal = {Journal of the American Statistical Association},
   Volume = {96},
   Number = {456},
   Pages = {1348-1360},
      Year = {2001} }



@article{
fan04,
   Author = {Fan, J. Q. and Peng, H.},
   Title = {Nonconcave penalized likelihood with a diverging number of parameters},
   Journal = {Annals of Statistics},
   Volume = {32},
   Number = {3},
   Pages = {928-961},
      Year = {2004} }



@article{
friedman04,
   Author = {Friedman, N.},
   Title = {Inferring cellular networks using probabilistic graphical models},
   Journal = {Science},
   Volume = {303},
   Number = {5659},
   Pages = {799-805},
      Year = {2004} }



@article{
gardner03,
   Author = {Gardner, T. S. and di Bernardo, D. and Lorenz, D. and Collins, J. J.},
   Title = {Inferring genetic networks and identifying compound mode of action via expression profiling},
   Journal = {Science},
   Volume = {301},
   Number = {5629},
   Pages = {102-105},
      Year = {2003} }



@article{
gelman96,
   Author = {Gelman, A. and Bois, F. and Jiang, J. M.},
   Title = {Physiological pharmacokinetic analysis using population modeling and informative prior distributions},
   Journal = {Journal of the American Statistical Association},
   Volume = {91},
   Number = {436},
   Pages = {1400-1412},
      Year = {1996} }



@article{
ghosal00,
   Author = {Ghosal, S. and Ghosh, J. K. and Van der Vaart, A. W.},
   Title = {Convergence rates of posterior distributions},
   Journal = {Annals of Statistics},
   Volume = {28},
   Number = {2},
   Pages = {500-531},
      Year = {2000} }



@article{
ghosal07,
   Author = {Ghosal, S. and Van Der Vaart, A.},
   Title = {Convergence rates of posterior distributions for noniid observations},
   Journal = {Annals of Statistics},
   Volume = {35},
   Number = {1},
   Pages = {192-223},
      Year = {2007} }



@article{
greenshtein04,
   Author = {Greenshtein, E. and Ritov, Y.},
   Title = {Persistence in high-dimensional linear predictor selection and the virtue of overparametrization},
   Journal = {Bernoulli},
   Volume = {10},
   Number = {6},
   Pages = {971-988},
      Year = {2004} }



@article{
haario01,
   Author = {Haario, H. and Saksman, E. and Tamminen, J.},
   Title = {An adaptive Metropolis algorithm},
   Journal = {Bernoulli},
   Volume = {7},
   Number = {2},
   Pages = {223-242},
      Year = {2001} }



@article{
hall87,
   Author = {Hall, P. and Marron, J. S.},
   Title = {ESTIMATION OF INTEGRATED SQUARED DENSITY DERIVATIVES},
   Journal = {Statistics \& Probability Letters},
   Volume = {6},
   Number = {2},
   Pages = {109-115},
      Year = {1987} }



@article{
triebel05,
   Author = {Haroske, D. A. and Triebel, H.},
   Title = {Wavelet bases and entropy numbers in weighted function spaces},
   Journal = {Mathematische Nachrichten},
   Volume = {278},
   Number = {1-2},
   Pages = {108-132},
      Year = {2005} }



@article{
hirose08,
   Author = {Hirose, Osamu and Yoshida, Ryo and Imoto, Seiya and Yamaguchi, Rui and Higuchi, Tomoyuki and Charnock-Jones, D. Stephen and Print, Cristin and Miyano, Satoru},
   Title = {Statistical inference of transcriptional module-based gene networks from time course gene expression profiles by using state space models},
   Journal = {Bioinformatics},
   Volume = {24},
   Number = {7},
   Pages = {932-942},
      Year = {2008} }



@article{
hoff07,
   Author = {Hoff, Peter D.},
   Title = {Model Averaging and Dimension Selection for the Singular Value Decomposition},
   Journal = {Journal of the American Statistical Association},
   Volume = {102},
   Pages = {674-685},
   Note = {[1]
doi:10.1198/016214506000001310},
      Year = {2007} }



@article{
huangma08,
   Author = {Huang, J. and Horowitz, J. L. and Ma, S. G.},
   Title = {Asymptotic properties of bridge estimators in sparse high-dimensional regression models},
   Journal = {Annals of Statistics},
   Volume = {36},
   Number = {2},
   Pages = {587-613},
      Year = {2008} }



@article{
huangma06,
   Author = {Huang, J. and Ma, S. G. and Zhang, C.H.},
   Title = {Adaptive lasso for sparse high-dimensional regression models},
   Journal = {Tech. rep., The University of Iowa},
   Volume={},
   Number={},
   Pages={},
      Year = {2006} }



@article{
huangfan99,
   Author = {Huang, L. S. and Fan, J. Q.},
   Title = {Nonparametric estimation of quadratic regression functionals},
   Journal = {Bernoulli},
   Volume = {5},
   Number = {5},
   Pages = {927-949},
      Year = {1999} }



@article{
hunter04,
   Author = {Hunter, D. R. and Lange, K.},
   Title = {A tutorial on MM algorithms},
   Journal = {American Statistician},
   Volume = {58},
   Number = {1},
   Pages = {30-37},
      Year = {2004} }



@article{
jaakkola94,
   Author = {Jaakkola, T. and Jordan, M. I. and Singh, S. P.},
   Title = {ON THE CONVERGENCE OF STOCHASTIC ITERATIVE DYNAMIC-PROGRAMMING ALGORITHMS},
   Journal = {Neural Computation},
   Volume = {6},
   Number = {6},
   Pages = {1185-1201},
      Year = {1994} }



@article{
johnstone05,
   Author = {Johnstone, I. M. and Silverman, B. W.},
   Title = {Empirical Bayes selection of wavelet thresholds},
   Journal = {Annals of Statistics},
   Volume = {33},
   Number = {4},
   Pages = {1700-1752},
      Year = {2005} }



@article{
kleijn06,
   Author = {Kleijn, B. J. K. and Van der Vaart, A. W.},
   Title = {Misspecification in infinite-dimensional Bayesian statistics},
   Journal = {Annals of Statistics},
   Volume = {34},
   Number = {2},
   Pages = {837-877},
      Year = {2006} }



@article{
laurent96,
   Author = {Laurent, B.},
   Title = {Efficient estimation of integral functionals of a density},
   Journal = {Annals of Statistics},
   Volume = {24},
   Number = {2},
   Pages = {659-681},
      Year = {1996} }



@article{
laurent97,
   Author = {Laurent, B.},
   Title = {Estimation of integral functionals of a density and its derivatives},
   Journal = {Bernoulli},
   Volume = {3},
   Number = {2},
   Pages = {181-211},
      Year = {1997} }



@article{
lawrence05,
   Author = {Lawrence, Neil},
   Title = {Probabilistic Non-linear Principal Component Analysis with Gaussian Process Latent Variable Models},
   Journal = {J. Mach. Learn. Res.},
   Volume = {6},
   Pages = {1783-1816},
   Keywords = {pca},
   Year = {2005} }



@article{
meinshausen06,
   Author = {Meinshausen, N. and Buhlmann, P.},
   Title = {High-dimensional graphs and variable selection with the Lasso},
   Journal = {Annals of Statistics},
   Volume = {34},
   Number = {3},
   Pages = {1436-1462},
      Year = {2006} }



@article{
nam07,
   Author = {Nam, D. and Yoon, S. H. and Kim, J. F.},
   Title = {Ensemble learning of genetic networks from time-series expression data},
   Journal = {Bioinformatics},
   Volume = {23},
   Number = {23},
   Pages = {3225-3231},
      Year = {2007} }




@article{
nickl07,
   Author = {Nickl, R. and Potscher, B. M.},
   Title = {Bracketing metric entropy rates and empirical central limit theorems for function classes of Besov- and Sobolev-type},
   Journal = {Journal of Theoretical Probability},
   Volume = {20},
   Number = {2},
   Pages = {177-199},
      Year = {2007} }



@article{
ramsay07,
   Author = {Ramsay, J. O. and Hooker, G. and Campbell, D. and Cao, J.},
   Title = {Parameter estimation for differential equations: a generalized smoothing approach},
   Journal = {Journal of the Royal Statistical Society Series B-Statistical Methodology},
   Volume = {69},
   Pages = {741-770},
      Year = {2007} }



@article{
rosset07,
   Author = {Rosset, S. and Zhu, J.},
   Title = {Piecewise linear regularized solution paths},
   Journal = {Annals of Statistics},
   Volume = {35},
   Number = {3},
   Pages = {1012-1030},
      Year = {2007} }



@article{
schwartz65,
   Author = {Schwartz, L.},
   Title = {On Bayes Procedures},
   Journal = {Z. Wahrsch. Verw. Gabiete},
   Volume = {4},
   Pages = {10-26},
      Year = {1965} }



@article{
shenwong01,
   Author = {Shen, X. T. and Wasserman, L.},
   Title = {Rates of convergence of posterior distributions},
   Journal = {Annals of Statistics},
   Volume = {29},
   Number = {3},
   Pages = {687-714},
      Year = {2001} }



@article{
simon01,
   Author = {Simon, I. and Barnett, J. and Hannett, N. and Harbison, C. T. and Rinaldi, N. J. and Volkert, T. L. and Wyrick, J. J. and Zeitlinger, J. and Gifford, D. K. and Jaakkola, T. S. and Young, R. A.},
   Title = {Serial regulation of transcriptional regulators in the yeast cell cycle},
   Journal = {Cell},
   Volume = {106},
   Number = {6},
   Pages = {697-708},
      Year = {2001} }



@article{
spellman98,
   Author = {Spellman, P. T. and Sherlock, G. and Zhang, M. Q. and Iyer, V. R. and Anders, K. and Eisen, M. B. and Brown, P. O. and Botstein, D. and Futcher, B.},
   Title = {Comprehensive identification of cell cycle-regulated genes of the yeast Saccharomyces cerevisiae by microarray hybridization},
   Journal = {Molecular Biology of the Cell},
   Volume = {9},
   Number = {12},
   Pages = {3273-3297},
      Year = {1998} }



@article{
teixeira06,
   Author = {Teixeira, M. C. and Monteiro, P. and Jain, P. and Tenreiro, S. and Fernandes, A. R. and Mira, N. P. and Alenquer, M. and Freitas, A. T. and Oliveira, A. L. and Sa-Correia, I.},
   Title = {The YEASTRACT database: a tool for the analysis of transcription regulatory associations in Saccharomyces cerevisiae},
   Journal = {Nucleic Acids Research},
   Volume = {34},
   Pages = {D446-D451},
      Year = {2006} }



@article{
tibshirani96,
   Author = {Tibshirani, R.},
   Title = {Regression shrinkage and selection via the Lasso},
   Journal = {Journal of the Royal Statistical Society Series B-Methodological},
   Volume = {58},
   Number = {1},
   Pages = {267-288},
      Year = {1996} }



@article{
tipping99,
   Author = {Tipping, Michael E. and Bishop, Christopher M.},
   Title = {Mixtures of Probabilistic Principal Component Analyzers},
   Journal = {Neural Computation},
   Volume = {11},
   Number = {2},
   Pages = {443-482},
      Year = {1999} }



@article{
tippingpca99,
   Author = {Tipping, Michael E. and Bishop, Christopher M.},
   Title = {Probabilistic Principal Component Analysis},
   Journal = {Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
   Volume = {61},
   Number = {3},
   Pages = {611-622},
      Year = {1999} }



@article{
tsitsiklis94,
   Author = {Tsitsiklis, J. N.},
   Title = {ASYNCHRONOUS STOCHASTIC-APPROXIMATION AND Q-LEARNING},
   Journal = {Machine Learning},
   Volume = {16},
   Number = {3},
   Pages = {185-202},
      Year = {1994} }



@article{
varah82,
   Author = {Varah, J. M.},
   Title = {A SPLINE LEAST-SQUARES METHOD FOR NUMERICAL PARAMETER-ESTIMATION IN DIFFERENTIAL-EQUATIONS},
   Journal = {Siam Journal on Scientific and Statistical Computing},
   Volume = {3},
   Number = {1},
   Pages = {28-46},
      Year = {1982} }



@article{
walker03,
   Author = {Walker, S.},
   Title = {On sufficient conditions for Bayesian consistency},
   Journal = {Biometrika},
   Volume = {90},
   Number = {2},
   Pages = {482-488},
      Year = {2003} }



@article{
walker04,
   Author = {Walker, S.},
   Title = {New approaches to Bayesian consistency},
   Journal = {Annals of Statistics},
   Volume = {32},
   Number = {5},
   Pages = {2028-2043},
      Year = {2004} }



@article{
walker07,
   Author = {Walker, S.  and Lijoi, A.  and Pr\"unster, I.},
   Title = {On rates of convergence for posterior distributions in infinite-dimensional models},
   Journal = {Annals of Statistics},
   Volume = {35},
   Number = {2},
   Pages = {738-746},
      Year = {2007} }





@article{
webb96,
   Author = {Webb, Andrew R.},
   Title = {An approach to non-linear principal components analysis using radially symmetric kernel functions},
   Journal = {Statistics and Computing},
   Volume = {6},
   Number = {2},
   Pages = {159-168},
   Note = {10.1007/BF00162527},
   Abstract = {An approach to non-linear principal components using radially symmetric kernel basis functions is described. The procedure consists of two steps: a projection of the data set to a reduced dimension using a non-linear transformation whose parameters are determined by the solution of a generalized symmetric eigenvector equation. This is achieved by demanding a maximum variance transformation subject to a normalization condition (Hotelling's approach) and can be related to the homogeneity analysis approach of Gifi through the minimization of a loss function. The transformed variables are the principal components whose values define contours, or more generally hypersurfaces, in the data space. The second stage of the procedure defines the fitting surface, the principal surface, in the data space (again as a weighted sum of kernel basis functions) using the definition of self-consistency of Hastie and Stuetzle. The parameters of this principal surface are determined by a singular value decomposition and crossvalidation is used to obtain the kernel bandwidths. The approach is assessed on four data sets.},
      Year = {1996} }



@article{
yu04,
   Author = {Yu, J. and Smith, V. A. and Wang, P. P. and Hartemink, A. J. and Jarvis, E. D.},
   Title = {Advances to Bayesian network inference for generating causal networks from observational biological data},
   Journal = {Bioinformatics},
   Volume = {20},
   Number = {18},
   Pages = {3594-3603},
      Year = {2004} }



@article{
zhao00,
   Author = {Zhao, L. H.},
   Title = {Bayesian aspects of some nonparametric problems},
   Journal = {Annals of Statistics},
   Volume = {28},
   Number = {2},
   Pages = {532-552},
      Year = {2000} }



@article{
zhaoyu06,
   Author = {Zhao, P. and Yu, B.},
   Title = {On model selection consistency of Lasso},
   Journal = {Journal of Machine Learning Research},
   Volume = {7},
   Pages = {2541-2563},
   Note = {Zhao, Peng Yu, Bin},
      Year = {2006} }



@article{
zou06,
   Author = {Zou, H.},
   Title = {The adaptive lasso and its oracle properties},
   Journal = {Journal of the American Statistical Association},
   Volume = {101},
   Number = {476},
   Pages = {1418-1429},
      Year = {2006} }




